HPGNN: Using Hierarchical Graph Neural Networks for Outdoor Point Cloud Processing

Inspired by recent improvements in point cloud processing for autonomous navigation, we focus on using hierarchical graph neural networks for processing and feature learning over large-scale outdoor LiDAR point clouds. We observe that existing GNN based methods fail to overcome challenges of scale and irregularity of points in outdoor datasets. Addressing the need to preserve structural details while learning over a larger volume efficiently, we propose Hierarchical Point Graph Neural Network (HPGNN). It learns node features at various levels of graph coarseness to extract information. This enables to learn over a large point cloud while retaining fine details that existing point-level graph networks struggle to achieve. Connections between multiple levels enable a point to learn features in multiple scales, in a few iterations. We design HPGNN as a purely GNN-based approach, so that it offers modular expandability as seen with other point-based and Graph network baselines. To illustrate the improved processing capability, we compare previous point based and GNN models for semantic segmentation with our HPGNN, achieving a significant improvement for GNNs (+36.7 mIoU) on the SemanticKITTI dataset.

==> tables/result3.tex <==
\begin{table*}[!t]
\caption{mIoU scores compared with single scan semantic segmentation on nuScenes-Lidarseg test set. Our model is compared with second generation models employing point networks or graph networks as their underlying architecture.}
\label{tab:result3}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|cccccccccccccccc|} 
\hline
Method & mIoU & 
\begin{sideways}Barrier\end{sideways} & 
\begin{sideways}Bicycle\end{sideways} & 
\begin{sideways}Bus\end{sideways} & 
\begin{sideways}Car\end{sideways} & 
\begin{sideways}Constr. veh.\end{sideways} & \begin{sideways}Motorcycle\end{sideways} & \begin{sideways}Pedestrian\end{sideways} & 
\begin{sideways}Traffic cone\end{sideways} & \begin{sideways}Trailer\end{sideways} & 
\begin{sideways}Truck\end{sideways} & 
\begin{sideways}Drivable\end{sideways} & 
\begin{sideways}Other flat\end{sideways} & \begin{sideways}Sidewalk\end{sideways} & \begin{sideways}Terrain\end{sideways} & 
\begin{sideways}Man made\end{sideways} & 
\begin{sideways}Vegetation\end{sideways} \\ 
\hline
% SqueezeSegv3 \cite{xu2021squeezesegv3} & 55.9 & 92.5 & 38.7 & 36.5 & 29.6 & 33.0 & 45.6 & 46.2 & 20.1 & 91.7 & 63.4 & 74.8 & 26.4 & 89.0 & 59.4 & 82.0 & 58.7 & 65.4 & 49.6 & 58.9 \\
% SalsaNext \cite{cortinhal2020salsanext}  & 59.5 & 91.9 & 48.3 & 38.6 & 38.9 & 31.9 & 60.2 & 59.0 & 19.4 & 91.7 & 63.7 & 75.8 & 29.1 & 90.2 & 64.2 & 81.8 & 63.6 & 66.5 & 54.3 & 62.1 \\ 

%\hline
 
%\hline
%RandLANet \cite{huRandlanet} & 53.9 & 94.2 & 26.0 & 25.8 & 40.1 & 38.9 & 49.2 & 48.2 & 7.2 & 90.7 & 60.3 & 73.7 & 20.4 & 86.9 & 56.3 & 81.4 & 61.3 & 66.8 & 49.2 & 47.7 \\
Polarnet \cite{PolarnetZhang2020} & 69.4 & 72.2 & 16.8 & 77.0 & 86.5 & 51.1 & 69.7 & 64.8 & 54.1 & 69.7 & 63.5 & 96.6 & 67.1 & 77.7 & 72.1 & 87.1 & 84.5 \\

Cylinder3D \cite{ZhuCylindricalAsym} & 77.2 & 82.8 & 29.8 & 84.3 & 89.4 & 63.0 & 79.3 & 77.2 & 73.4 & 84.6 & 69.1 & 97.7 & 70.2 & 80.3 & 75.5 & 90.4 & 87.6 \\

AMVNet \cite{Liong2020AMVNetAM} & 77.3 & 80.6 & 32.0 & 81.7 & 88.9 & 67.1 & 84.3 & 76.1 & 73.5 & 84.9 & 67.3 & 97.5 & 67.4 & 79.4 & 75.5 & 91.5 & 88.7 \\

SPVNAS \cite{tang2020spvnas} & 77.4 & 80.0 & 30.0 & 91.9 & 90.8 & 64.7 & 79.0 & 75.6 & 70.9 & 81.0 & 74.6 & 97.4 & 69.2 & 80.0 & 76.1 & 89.3 & 87.1 \\

AF2S3Net \cite{cheng2021af2s3net} & 78.3 & 78.9 & 52.2 & 89.9 & 84.2 & 77.4 & 74.3 & 77.3 & 72.0 & 83.9 & 73.8 & 97.1 & 66.5 & 77.5 & 74.0 & 87.7 & 86.8 \\

SPVCNN++ \cite{tang2020spvnas} & 81.1 & 86.4 & 43.1 & 91.9 & 92.2 & 75.9 & 75.7 & 83.4 & 77.3 & 86.8 & 77.4 & 97.7 & 71.2 & 81.1 & 77.2 & 91.7 & 89.0\\ 

\hline
\multicolumn{18}{c}{}\\
\hline
%SPGraph \cite{LandrieuSuperPoint} & 17.4 & 49.3 & 0.2 & 0.2 & 0.1 & 0.8 & 0.3 & 2.7 & 0.1 & 45.0 & 0.6 & 28.5 & 0.6 & 64.3 & 20.8 & 48.9 & 27.2 & 24.6 & 15.9 & 0.8 \\
\textbf{HPGNN - Ours} \\
\hline
\end{tabular}}
\end{table*}
